Optimistic Online Mirror Descent for Bridging Stochastic and Adversarial Online Convex Optimization

Stochastically Extended Adversarial (SEA) model is introduced by Sachs et al. [2022] as an interpolation between stochastic and adversarial online convex optimization. Under the smoothness condition, they demonstrate that the expected regret of optimistic follow-the-regularized-leader (FTRL) depends on the cumulative stochastic variance $\sigma_{1:T}^2$ and the cumulative adversarial variation $\Sigma_{1:T}^2$ for convex functions. They also provide a slightly weaker bound based on the maximal stochastic variance $\sigma_{\max}^2$ and the maximal adversarial variation $\Sigma_{\max}^2$ for strongly convex functions. Inspired by their work, we investigate the theoretical guarantees of optimistic online mirror descent (OMD) for the SEA model. For convex and smooth functions, we obtain the same $\mathcal{O}(\sqrt{\sigma_{1:T}^2}+\sqrt{\Sigma_{1:T}^2})$ regret bound, without the convexity requirement of individual functions. For strongly convex and smooth functions, we establish an $\mathcal{O}((\sigma_{\max}^2 + \Sigma_{\max}^2) \log (\sigma_{1:T}^2+\Sigma_{1:T}^2))$ bound, better than their $\mathcal{O}((\sigma_{\max}^2 + \Sigma_{\max}^2) \log T)$ result. For exp-concave and smooth functions, we achieve a new $\mathcal{O}(d\log(\sigma_{1:T}^2+\Sigma_{1:T}^2))$ bound. Owing to the OMD framework, we broaden our work to study dynamic regret minimization and scenarios where the online functions are non-smooth. We establish the first dynamic regret guarantee for the SEA model with convex and smooth functions, which is more favorable than static regret bounds in non-stationary scenarios. Furthermore, to deal with non-smooth and convex functions in the SEA model, we propose novel algorithms building on optimistic OMD with an implicit update, which provably attain static regret and dynamic regret guarantees without smoothness conditions.

==> sections/problem_setup.tex <==
%!TEX root = ../OMD4SEA_arxiv.tex
\section{Problem Setup and Existing Results}
\label{sec:problem}
Besides, the following standard assumptions for online convex optimization are required~\citep{Intro:Online:Convex,Modern:Online:Learning}.
\begin{ass}[boundedness of gradient norms]\label{ass:3} The gradients of all the individual functions are bounded by $G$, i.e.~for all $t \in [T]$, we have $\max_{\x \in \X}\|\nabla f_t(\x)\|_2 \leq G$.
\end{ass}
\begin{ass}[domain boundedness]\label{ass:4} The domain $\X$ contains the origin $\mathbf{0}$, and the diameter of $\X$ is bounded by $D$, i.e.,~for all $\x,\y \in \X$, we have $\|\x -\y\|_2 \leq D$.
\end{ass}

\paragraph{Existing Results.} With the smoothness of expected loss functions, \citet{OCO:Between} establish a series of results for the SEA model, including convex functions and strongly convex functions. In the case of convex and smooth functions, they prove an $\O(\sqrt{\sigma_{1:T}^2}+\sqrt{\Sigma_{1:T}^2})$ regret bound of optimistic FTRL. Note that they require the individual functions $\{f_t\}_{t=1}^T$ to be convex, which is relatively strict. When facing the adversarial setting, we have $\sigma_t^2 = 0$ for all $t$ and $\Sigma_{1:T}^2$ is equivalent to $V_T$, so the bound implies $\O(\sqrt{V_T})$ regret matching the result of~\citet{Gradual:COLT:12}, which also reduces to the $\O(\sqrt{T})$ bound in the worst case~\citep{zinkevich-2003-online}. In the SCO setting, we have $\Sigma_{1:T}^2 = 0$ and $\sigma_t = \sigma$ for all $t$, where $\sigma$ denotes the variance of stochastic gradients. Then they obtain $\O(\sigma \sqrt{T})$ regret, leading to an $\O(\sigma/\sqrt{T})$ excess risk bound through the standard online-to-batch conversion~\citep{TIT04:Bianchi}.

To investigate the strongly convex case, they make an additional assumption about the \emph{maximum value} of stochastic variance and adversarial variation.
\begin{ass}[maximal stochastic variance and adversarial variation]\label{ass:sigma}
All the variances of realizable gradients are at most $\sigma_{\max}^2$, and all the adversarial variations are upper bounded by $\Sigma_{\max}^2$, i.e., $\forall t \in [T]$, it holds that $\sigma_{t}^2 \leq \sigma_{\max}^2$ and $\sup_{\x \in \X} \|\nabla F_t(\x)- \nabla F_{t-1}(\x)\|_2^2 \leq \Sigma_{\max}^2$.
\end{ass}
Based on Assumption~\ref{ass:sigma}, \citet{OCO:Between} prove an $\O((\sigma_{\max}^2 + \Sigma_{\max}^2) \log T)$ expected regret bound of optimistic FTRL for $\lambda$-strongly convex and smooth functions. Considering the adversarial setting, we have $\sigma_{\max}^2 = 0$ and $\Sigma_{\max}^2 \leq 4G^2$, so their bound implies an $\O(\log T)$ regret bound. We note that unlike in the convex and smooth case, their expected regret bound fails to recover the $\O(\log V_T)$ gradient-variation bound~\citep{ICML:2022:Zhang}. In the SCO setting, we have $\Sigma_{\max}^2 = 0$ and $\sigma_{\max}^2 = \sigma^2$. Therefore, their result brings an $\O([\sigma^2 \log T]/T)$ excess risk bound through online-to-batch conversion.
